Choco-Q: Commute Hamiltonian-based QAOA for Constrained Binary Optimization

Constrained binary optimization aims to find an optimal assignment to minimize or maximize the objective meanwhile satisfying the constraints, which is a representative NP problem in various domains, including transportation, scheduling, and economy. Quantum approximate optimization algorithms (QAOA) provide a promising methodology for solving this problem by exploiting the parallelism of quantum entanglement. However, existing QAOA approaches based on penalty-term or Hamiltonian simulation fail to thoroughly encode the constraints, leading to extremely low success rate and long searching latency. This paper proposes Choco-Q, a formal and universal framework for constrained binary optimization problems, which comprehensively covers all constraints and exhibits high deployability for current quantum devices. The main innovation of Choco-Q is to embed the commute Hamiltonian as the driver Hamiltonian, resulting in a much more general encoding formulation that can deal with arbitrary linear constraints. Leveraging the arithmetic features of commute Hamiltonian, we propose three optimization techniques to squeeze the overall circuit complexity, including Hamiltonian serialization, equivalent decomposition, and variable elimination. The serialization mechanism transforms the original Hamiltonian into smaller ones. Our decomposition methods only take linear time complexity, achieving end-to-end acceleration. Experiments demonstrate that Choco-Q shows more than 235$\times$ algorithmic improvement in successfully finding the optimal solution, and achieves 4.69$\times$ end-to-end acceleration, compared to prior QAOA designs.

==> hpcatemplate.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  


==> section/4_opt1.tex <==

\section{Optimiazation on Hamiltonian Construction}
The construction process of a Hamiltonian commute can be time-consuming and space-consuming due to the high overhead of linear equation solving and massive tensor operations. 
To minimize classical computation overhead, we improve the linear equation solver by leveraging the solution pattern in a specific problem and avoiding the numeric calculation of the Hamiltonian. Specifically, we give an analytical method for the commute Hamiltonian construction~(Section~\ref{subsec:analyticaltheory}), reducing the overhead from cubic to linear complexity. Section~\ref{subsec:analyticalimpl} gives a tiny example to illustrate this analytical method for linear equation solving. Finally, instead of computing the whole tensor format of the commute Hamiltonian, we send the solutions from the analytical solver to the Hamiltonian simulation since the solutions can uniquely represent the commute Hamiltonian.

\subsection{Analytical Construction Formulation}
\label{subsec:analyticaltheory}
The high classical computation overhead of constructing the commute Hamiltonian comes from the numeric computation of the specific form of Hamiltonian. For example, an arbitrary numeric linear solver needs $O(n^3)$ complexity to get all solutions of the linear equation $C\vec{u}=0$. However, this equation is quite special since the solutions are in a discrete set $\{1,-1,0\}^n$. Besides, we observed that in most applications, the constraints always have the same pattern independent of the scale of the problem. This inspires us to find an analytical approach to deal with the equation. Thus, We propose the following theory to solve the linear equation analytically.

\begin{lemma}\label{theorem:linearsolving}
    Given a constrained equation $C\vec{u}=0$ with symbolic representation, we can solve the equation in $O(n)$ complexity by analytical solution, where $n$ is the dimension of $\vec{u}$.
\end{lemma}
\begin{proof}
    
\end{proof}

Here, A symbolic representation is like $\sum_{j}^n x_j=0$, which means the pattern of Hamiltonian construction equation $C\vec{u}=0$ is not changed with the scale $n$ of the problem. Since constrained binary optimization always comes from modeling the real world in a scalable way, the constrained equation is easily represented in a symbolic form. 
Thus, we can solve the constrained equation symbolically, which provides an exact solution. We can apply the symbolic solution for a specific problem with a known scale to get the solution in $O(n)$ complexity. 

\subsection{Analytical Construction Implementation}
\label{subsec:analyticalimpl}
Without losing generality, we take the following example to illustrate analytical solving.
\begin{small}
\begin{equation}
\begin{aligned}
    \sum_{j}^n y_{ij}&=0\quad &\forall i \in \{1,\cdots,m\}&\\
\end{aligned}
\label{eq:lineareqexp1}
\end{equation}
\end{small}
\begin{small}
\begin{equation}
\begin{aligned}
    x_j - y_{ij} &= 0\quad&\forall i \in \{1,\cdots,m\}&\;\forall j \in \{1,\cdots,n\}
\end{aligned}
\label{eq:lineareqexp2}
\end{equation}
\end{small}
This constraint contains two equations with total $mn+n$ variables.
The core idea is to represent other variables with independent variables. Here, the independent variables mean that the constraint equations do not make restrictions on their assignment. We try to select $y_{mj},\forall j \in \in \{1,\cdots,n\}$ as independent variables because they are only constrained by Equation~\ref{eq:lineareqexp1}, \ie, $\sum_{j}^n y_{mj} = 0$. Thereby, we can set $y_{mj} \; \forall j \in \{1,\cdots,n-1\}$ as independent variables and $y_{mn}$ is determined by $y_{mn}= -\sum_{j}^{n-1} y_{mj}$.
Setting $i =m$ in Equation~\ref{eq:lineareqexp2} gives $x_j =y_{mj},\quad \forall j \in \{1,\cdots,n\}$, which is the representation of $x_j$. Replacing $x_j$
Equation~\ref{eq:lineareqexp2} for $i\neq m$ by $x_j =y_{mj}$ gives $y_{ij}=y_{mj}$, which is the representation of $y_{ij}$. In a word, we find the expression of all variables represented by $n-1$ independent variable $y_{mj},\forall j  \in \{1,\cdots,n-1\}$. The basic solution is given by setting one of the independent variables as $1$ and setting the other as $0$. In this case, there are $n-1$ basic solutions, and $k$-th solution is obtained by setting $y_{mk}=1$ and other variables $y_{mj}=0,\forall j\neq k$. 
The same idea can be applied to other problems with symbolical constraint formulation. For more specific problems, we provide the analytical solution in Section~\ref{sec:casestudy}.



==> section/5_casestudy.tex <==
\section{Case Study}\label{sec:casestudy}
\subsection{Facility Location Problem}



The facility location problem (FLP) is an optimization problem that is widely studied in operations research and logistics~\cite{farahani2009facility}. It addresses where to locate facilities (such as warehouses, factories, or service centers) to minimize costs while meeting the supply demands. For simplicity, we focus on the uncapacitated FLP~\cite{cornuejols1983uncapicitated}, which allows facilities to have unlimited capacity and thus can serve unlimited demands. 
This problem can be formulated as a constrained binary optimization as shown in Figure~\ref{fig:casestury}~(a). We use $ o_f $ to indicate whether facility $ f \in \mathcal{F}$ is open and use $ s_{d,f} $ to denote whether demand $ d \in \mathcal{D} $ is supplied from facility $ f $. The constraints include:
\begin{itemize}[leftmargin=*]
    \item \textit{Each demand can only be assigned to one facility}, which is formulated by restricting the summation of $s_{d,f}$ to 1. For example, in Figure~\ref{fig:casestury}~(a), demand No.1 has been supplied by facility No.1 ($s_{1,1}=1$), thereby, other facilities like facility No.2 cannot supply demand $1$ ($s_{1,2}=0$). 
    \item \textit{An unopened facility cannot supply any demand.} This constraint is formulated as $s_{d,f}$ cannot exceed $o_{f}$. In other words, when $o_{f}$ is 0, $s_{d,f}$ must be 0. For instance, since facility No.2 is not opened ($o_2=0$), it cannot supply any demand. 
    Since this constraint is not equality, we add ancillary binary variables $a_{d,f}$ to make it into equality format. When $o_{f}$ is 1, $s_{d,f}$ can be 0 or 1 while $a_{d,f}$ is 1 or 0, respectively. When $o_f$ is 0, $s_{d,f}$ and $a_{d,f}$ must be 0. 
\end{itemize}
The cost of opening facilities and supplying demand are pre-obtained, which are defined as $co_{f}$ and $cs_{d,f}$, respectively. The objective is to find which facilities should open $o_f$ and the assignment strategy $s_{d,f}$ to minimize the total cost. For example, when we chose to open facility $1$ to supply demand $1$, the supplying cost is $cs_{1,1}=1.5$, and the opening cost is $co_{1}=0.5$, leading to a total cost of 2. For an FLP with $|\mathcal{F}|$ facilities and $|\mathcal{D}|$ demands, it has $2|\mathcal{F}|\cdot|\mathcal{D}|+|\mathcal{F}|$ variables with $|\mathcal{D}|+|\mathcal{F}|\cdot |\mathcal{D}|$ constraints.
% Since the solution set $\Delta$ size is the size of variables subtracted by the size of constraints, which is $FD+F-D$. Our sequence commute Hamiltonian formulation thus has $FD+F-D$ terms. After decomposing the Hamiltonian term by phase gate, the whole circuit depth is $(FD+F-D)\cdot (FD+ 16D)\cdot L$, where $FD+ 16D$ is the depth of a local Hamiltonian simulation circuit and $L$ is the number of repeated layers ($\le 5$).

\subsection{Graph Coloring Problem}
The graph coloring problem (GCP) is a popular problem that has a broad range of practical applications~\cite{graphcoloring}, including scheduling~\cite{graphcoloringscheduling}, register allocation in compilers~\cite{registerallocation_graphcoloring}, and frequency assignment in wireless networks~\cite{park1996application}. 
The formulation of the graph coloring problem is shown in Figure~\ref{fig:casestury}~(b). Given an undirected graph $ \mathcal{G}= (\mathcal{V}, \mathcal{E}) $, where $ \mathcal{V} $ represents the set of vertices and $ \mathcal{E} $ denotes the set of edges, we use a binary variable $x_{i,k}$ to indicate whether vertex $i\in \mathcal{V} $ is colored by $ k \in \mathcal{C}$ ($\mathcal{C}$ is the set of all colors).
% the graph coloring problem is to assign a color $ k \in \mathcal{C}$ to each vertex $ i \in \mathcal{V} $,
The constraints include:
\begin{itemize}[leftmargin=*]
    \item \textit{Each vertex can only be colored by one color}, formulated in the same way as FLP. For example, the vertex No.1 has been colored by color No.2 ($x_{1,2}=1$), with colors No.1 and No.3 not used ($x_{1,1}=x_{1,3}=0$). 
    \item \textit{Adjacent vertexes cannot be colored with the same color.} This is formulated as that, for any color $k$, the summation of two connected variables $x_{i,k}$ cannot exceed one.
    For instance, vertex No.2 and No.3 are connected via an edge, and vertex No.3 has been colored by color No.1 ($x_{3,1}=1$), making vertex No.2 cannot be colored by color No.1 ($x_{2,1}=0$). 
    Since this constraint is not in an equality format, similarly, we add several ancillary binary variables.  
\end{itemize}
The GCP aims to minimize the total number of colors utilized, and the objective function is shown in Figure~\ref{fig:casestury}~(b). Totally, this problem has $|\mathcal{V}|\cdot |\mathcal{C}|+ |\mathcal{E}|\cdot |\mathcal{C}|$ variables and $|\mathcal{V}|+ |\mathcal{E}|\cdot |\mathcal{C}|$ constraints.


\subsection{K-Partition Problem}
The K-Partition problem (KPP) is also a graph-domain problem with many applications~\cite{wikipedia_partition_2024}, including load balancing~\cite{bhatele2011applying}, data clustering~\cite{zha2001bipartite}, and parallel processing~\cite{simon1991partitioning}.
The formulation of the K-Partition problem is shown in Figure~\ref{fig:casestury}~(c). Given an undirected graph $ \mathcal{G}= (\mathcal{V}, \mathcal{E}) $ and a positive integer $ K $, the K-Partition problem partitions the graph into $ K $ disjoint blocks $ \mathcal{B}$. Each block $k\in \mathcal{B}$ has a pre-obtained capacity $m_k$, and the weight of each edge is also pre-obtained, denoted as $w_{i,j}$. We use $x_{i,k}$ to indicate whether vertex $i$ is assigned to block $k$. The constraints including:
\begin{itemize}[leftmargin=*]
    \item \textit{Each vertex can only be housed in one block $k$}. The formulation is still the same as the other two problems. For example, vertex No.2 has been assigned to block No.2 ($x_{2,2}=1$), thereby, it cannot be assigned to block $1$ ($x_{2,1}=0$). 
    \item \textit{The size of vertexes in block $k$ equals its capacity $m_k$.} The size of vertexes in a block $k$ is calculated by the summation of all variables $x_{i,k}$ in the same block $k$. This summation must equal $m_k$.
    For instance, block No.1 can only contain two vertexes since its capacity $m_1$ is 2.   
\end{itemize}
The objective function is to maximize the summation of the cut weights. In the example of Figure~\ref{fig:casestury}~(c), vertex No.1 and No.2 are in different blocks. Thus, the edge (1,2) is cut. And the edge (3,2) is also cut. Their weight is 0.4 and 0.7, respectively. In this manner, the objective is 1.1. For the problem scale, the K-Partition problem has $|\mathcal{V}|\cdot|\mathcal{B}|$ variables and $|\mathcal{V}|+|\mathcal{B}|$ constraints in total.

==> section/5_complexity.tex <==
\section{\papername: Complexity analysis}


==> section/7_discussion.tex <==



\section{Discussion}
\label{sec:discussion}
\subsection{Parameter Initialization and Updating}
QAOA is very sensitive to the initial parameters. In unconstrained binary optimization, fine-tuned parameters can make QAOA converge to a good solution and reach a high success rate~\cite{redqaoa,frozenqubits}. However, when dealing with constrained binary optimization, even fine-tuned parameters also have a low probability of success. In our test,  in 10-qubit experiments, the fine-tuned QAOA can reach 10\% success probability at most. Our proposed algorithm is not sensitive to initial parameters since it uses hard constraints to ensure the high confidence of the solution. 


For parameter updating, \papername is not constrained by a specific parameter updating algorithm. The number of parameters in \papername aligns with the number of layers, which is below 5 in real applications with any scale. Since the size of the parameters is quite low, any parameter optimizer can overcome the optimization task. There may be an optimal optimizer specialized for \papername, and we leave it for future work.



\subsection{From Binary Optimization to Integer Programming}
The binary optimization problem is a representative branch of integer programming~\cite{williams2009integer} and plays a vital role in various applications. Theoretically, any integer programming can be formulated by binary optimization using the binary representation of the integer. However, this representation can introduce more auxiliary variables, which is not friendly in current mid-scale quantum computers. Besides, the representation makes the constraints more complicated than the binary case. The complex form of constraints may need a complex commute Hamiltonian, which cannot be efficiently implemented in the quantum hardware. We think there are two potential approaches to deal with integer programming using the quantum approach. One might investigate the commute Hamiltonian form of integer programming with binary representation and develop efficient decomposition for specific domains. Another approach might use a quantum adiabatic linear solver by encoding a normalized integer as the amplitude of the qubit state~\cite{adiabaticlinearquantum}. The commute Hamiltonian needs to be carefully designed to cope with the constraint.



==> section/deleted/3_overview.tex <==

\subsection{\papername: Overview}
% \hl{These are design challenges?}
To deal with the dilemma, we propose several methods to optimize the Hamiltonian construction and Hamiltonian simulation. Figure~\ref{fig:workflow} gives the workflow of  \papername, which follows the same procedure as illustrated in Section\ref{}. The Hamiltonian construction step receives the constraint matrix and objective function from the input problem and then constructs the objective Hamiltonian and driver Hamiltonian for simulation. The challenging task is the construction of the driver Hamiltonian. We design a specialized solver to speed up the solving of construction Equation~\ref{eq:lineareq}, which is based on our observation of the solution pattern for specific problem categories. We then find a new formulation of commute Hamiltonian. The new formulation of commute Hamiltonian provided a hardware-friendly commute Hamiltonian. We theoretically verified that this formulation is an efficient way to preserve the constraints in the problem and greatly reduce the cost of hardware deployments.

The constructed Hamiltonians must be decomposed into quantum circuits with elemental gates for simulation on a quantum device. We optimized the Hamiltonian simulation with a phase gate decomposer. This decomposer provides an exact decomposition for the simulated Hamiltonian and leverages multi-qubit phase gates to reduce the decomposed circuit depth on quantum hardware. We supported two hardware platforms, including neural atom computing devices and superconducting computers.



\begin{figure}[t]
    \centering
    \includegraphics[width=.90\linewidth]{pictures/sections/workflow.pdf}
    \vspace{-0.25cm}
    \caption{\papername workflow.}
    \label{fig:workflow}
    \vspace{-0.2cm}
\end{figure}


==> section/deleted/opt1.tex <==
% Note that in common case, $H_c(\vec{u})$ do not commutes with each other, thus 
% \begin{equation}
%     \small
%     e^{-i\beta_l H^d} \neq \Pi_{\vec{u}\in \Delta} e^{-i\beta_l  H_c(\vec{u})}
%     \notag
% \end{equation} 
% For example, in Equation~\eqref{eq:hdexample}, the Hamiltonian $H_c(\vec{u}^1)$ do not commute with $H_c(\vec{u}^2)$.
% % \begin{equation}
% % \begin{aligned}
% %     &H_c(\vec{u}^1) H_c(\vec{u}^2) \\
% %     &= (\sigma_1^{-1} \sigma_2^{+1} \sigma_3^{-1}
% %     +\sigma_1^{+1} \sigma_2^{-1} \sigma_3^{+1})
% %      ( \sigma_2^{-1} \sigma_4^{+1}+\sigma_2^{+1} \sigma_4^{-1} )\\
% %     &=  (\sigma_1^{-1} \sigma_2^{+1}\sigma_2^{-1} \sigma_3^{-1}\sigma_4^{+1}
% %     +\sigma_1^{+1} \sigma_2^{-1} \sigma_2^{+1}  \sigma_3^{+1} \sigma_4^{-1} )\\
% % \end{aligned}
% % \end{equation} 
% % \begin{equation}
% % \begin{aligned}
% %     &H_c(\vec{u}^1) H_c(\vec{u}^2) \\
% %     &= ( \sigma_2^{-1} \sigma_4^{+1}+\sigma_2^{+1} \sigma_4^{-1} )(\sigma_1^{-1} \sigma_2^{+1} \sigma_3^{-1}
% %     +\sigma_1^{+1} \sigma_2^{-1} \sigma_3^{+1})
% %      \\
% %     &=  (\sigma_1^{-1} \sigma_2^{-1}\sigma_2^{+1} \sigma_3^{-1}\sigma_4^{+1}
% %     +\sigma_1^{+1} \sigma_2^{+1} \sigma_2^{-1}  \sigma_3^{+1} \sigma_4^{-1} )\\
% % \end{aligned}
% % \end{equation} 
% % Thus 
% \begin{equation}
% \small
% \begin{aligned}
%     &[H_c(\vec{u}^1), H_c(\vec{u}^2)] = H_c(\vec{u}^1) H_c(\vec{u}^2) - H_c(\vec{u}^2) H_c(\vec{u}^1) \\
%     &= \sigma_2^z (\sigma_1^{-1} \sigma_4^{+1} \sigma_3^{-1}
%     - \sigma_1^{+1} \sigma_4^{-1} \sigma_3^{+1}) \neq 0 \notag
% \end{aligned}
% \end{equation} 
% Here, we omitted the intermediate calculations.
% \unfinished{For the unitary,}

==> section/deleted/opt2.tex <==
We first verify that $e^{-i\beta H_c(\vec{u})}$ has two orthogonal eigenstates $\ket{x^{+}}$ and $\ket{x^{-}}$,
    Their eigenvalues are $e^{- i\beta}$ and $e^{ i\beta}$, respectively. The eigenvalues of other orthogonal eigenstates are 1.  Firstly, we can easily verify that the Hamiltonian $H_c(\vec{u})$ has eigenstates $\ket{x^{\pm}}$ with eigenvalue $\pm 1$ and other eigenstates with eigenvalue 0.
    \begin{equation}
    \small
    \begin{aligned}
        H_c(\vec{u}) \ket{x^{\pm}}
        % &(\sigma_1^{u_1}\cdots \sigma_n^{u_n}+ \sigma_1^{-u_1}\cdots \sigma_n^{-u_n} ) \\
        % &(\frac{|v_1\cdots v_n \rangle \pm  |\bar{v}_1\cdots \bar{v}_n\rangle}{\sqrt{2}})\\
        % =& ( \frac{ \pm |\bar{v}_1\cdots \bar{v}_n\rangle + |v_1\cdots v_n \rangle}{\sqrt{2}}) 
        = \pm 1\cdot \ket{x^{\pm}}\\
    \end{aligned}
    \end{equation}
    \begin{equation}
    \small
    \begin{aligned}
        H_c(\vec{u}) \ket{other}= 0 \ket{other}\\
    \end{aligned}
    \end{equation}
    Since the exponential of a matrix has the same eigenvector but with an exponential value of eigenvalue, the unitary has the following eigenstate decomposition.
    \begin{equation}\small
    \begin{aligned}
        e^{-i\beta H_c(\vec{u})} \ket{x^{\pm}} =  e^{-i \beta \cdot \pm 1}\ket{x^{\pm}}= e^{\mp i\beta}\ket{x^{\pm}} \\
        e^{-i\beta H_c(\vec{u})} \ket{other} = e^{-i \beta \cdot 0 }\ket{other} = \ket{other}
    \end{aligned}
    \end{equation}

==> tab/benchcase.tex <==
\begin{tabular}{llllllllllll}
\toprule 
\multicolumn{4}{c}{\textbf{Facility location problem}~\cite{melo2009facilitylocation}} &
\multicolumn{4}{c}{\textbf{Graph coloring problem}~\cite{graphcoloring}} 
& \multicolumn{4}{c}{\textbf{K-partition problem}~\cite{kpartition}} \\ \cmidrule(lr){1-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12}
\textbf{Benchmark} &\textbf{\#Case} & \textbf{\#Var.} & \textbf{\#Con.}  
&\textbf{Benchmark} &\textbf{\#Case} & \textbf{\#Var.} & \textbf{\#Con.}  
&\textbf{Benchmark} &\textbf{\#Case} & \textbf{\#Var.} & \textbf{\#Con.}\\
\hline

 \FLNote{2}{1} & 100  & 6&3    & \GCNote{3}{1}{3} & 3 &12&9   & \KPNote{4}{3}{2}  & 100 &8&6     \\
  \FLNote{3}{2} & 100  &15&8   & \GCNote{3}{2}{3}& 3 &15&8    & \KPNote{6}{5}{3} & 100 &18&9    \\
 \FLNote{3}{3} & 100 & 21&12  & \GCNote{4}{2}{4}& 15 &24&12     & \KPNote{8}{7}{3} & 100 &24&11   \\
 \FLNote{4}{3} & 100 & 28&15  & \GCNote{4}{3}{4}& 20 &28&16     & \KPNote{9}{8}{3} & 100 &27&12   \\

\bottomrule
\multicolumn{12}{c}{\makecell[l]{2F-1D: two facilities and one demand. 3V-1E: a graph with three vertexes and one edge; \\4V-3E-2B: partitioning a graph, with four vertexes and three edges, into two blocks. }} \\

\end{tabular}

==> tab/benchmarks.tex <==

\begin{table}[t]
    \centering
    \caption{
   The benchmarks for evaluation.\label{tab:benchmark}
    }
    \renewcommand\arraystretch{1.05}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ll|llll}
    \toprule 
    \textbf{Domain} &\textbf{Benchmark} &\textbf{\#Case} & \textbf{\#Var.} & \textbf{\#Con.} & \textbf{Description } \\
    \hline
    \multirow{4}{*}{\makecell[c]{\textbf{FLP}\\~\cite{melo2009facilitylocation}}}  & \FLNote{2}{1} & 100  & 6&3 & \multirow{4}{*}{\makecell[l]{2F-1D means \\supplying one Demands\\ with two Facilities.}}   \\
     & \FLNote{3}{2} & 100  &15&8     \\
     & \FLNote{3}{3} & 100 & 21&12    \\
     & \FLNote{4}{3} & 100 & 28&15    \\
    \hline
    
    \multirow{4}{*}{\makecell[c]{\textbf{GCP}\\~\cite{graphcoloring}}} & \GCNote{3}{1}{3} & 100   &12&6  & \multirow{4}{*}{\makecell[l]{3V-1E means the graph \\ has three Vertexes \\ and one Edges. }}   \\
     & \GCNote{3}{2}{3}& 100   &15&9    \\ 
     & \GCNote{4}{2}{4}& 100 &24&12    \\
     & \GCNote{4}{3}{4}& 100 &28&16    \\
    \hline
    
    \multirow{4}{*}{\makecell[c]{\textbf{KPP}\\~\cite{kpartition}}} 
    & \KPNote{4}{3}{2}  & 100 &8&6 & \multirow{4}{*}{\makecell[l]{4V-3E-2B means the graph \\ with four Vertexes and \\ three Edges is partitioned\\ into two Blocks.}}      \\
     & \KPNote{6}{5}{3} & 100 &18&9    \\
     & \KPNote{8}{7}{3} & 100 &24&11   \\
     & \KPNote{9}{8}{3} & 100 &27&12   \\
    \hline
    \multirow{4}{*}{\makecell[c]{\textbf{JSP}\\~\cite{jobscheduling}}}  & J1: 2J-2M-3C & 100 & 7  & 4 & \multirow{4}{*}{\makecell[l]{2J-2M-3C means \\two Jobs is allocated to \\two Machines and the \\ machine Capacity is three.}}  \\
                                    & J2: 3J-3M-5C & 100 & 14 & 6 \\
                                    & J3: 3J-4M-6C & 100 & 18 & 7 \\
                                    & J4: 4J-5M-7C & 100 & 27 & 9 \\
    \hline
    \multirow{2}{*}{\makecell[c]{\textbf{TSP}\\~\cite{tsp}}}   & T1   : 4C & 100 & 11 & 8 & \multirow{2}{*}{\makecell[l]{4C means four Cities.}}  \\
                                       & T2: 5C & 100 & 27 & 16 \\
    \hline
    \multirow{3}{*}{\makecell[c]{\textbf{SCP}\\~\cite{setcovering}}}  & S1: 4S-4E & 100 & 9 & 4 & \multirow{3}{*}{\makecell[l]{4S-4E means covering \\ four Elements from the  \\ subsets of four Sets.}}  \\
                               & S2: 5S-5E & 100 & 12 & 5 \\
                               & S3: 6S-6E & 100 & 20 & 6 \\
                               % 4S-10C means that there are four sets with a total of ten coverings.
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.4cm}
    \end{table}
    
    

==> tab/breakdown.tex <==
\begin{table}[]
\centering
\footnotesize
\caption{XXXX}
\label{tab:breakdown}
% \renewcommand\arraystretch{1.4}
% \resizebox{\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
 & all & strategy 1 & strategy 2 & strategy 3 \\
\midrule
GC1 & 2.75 & 1.10 & 2.46 & 1.50 \\
GC2 & 3.22 & 1.09 & 2.75 & 1.57 \\
GC3 & 3.35 & 1.05 & 2.92 & 1.80 \\
CFA & 83.21 & 2.37 & 2.37 & 83.00 \\
BP & 7.00 & 7.00 & 3.02 & 1.53 \\
II & 6.82 & 3.05 & 1.88 & 1.01 \\
SP1 & 4.13 & 1.00 & 4.11 & 1.04 \\
SP2 & 3.65 & 1.00 & 3.18 & 2.64 \\
SP3 & 4.38 & 1.00 & 2.28 & 2.74 \\
SP4 & 8.89 & 1.00 & 5.73 & 2.69 \\
SP5 & 6.72 & 1.43 & 2.35 & 2.15 \\
Average & 12.19 & 1.92 & 3.00 & 9.24 \\
\bottomrule
\end{tabular}
% }
\end{table}

==> tab/noise-experiment.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{
Running time comparison between CDCL on Intel E5 CPU and HyQSAT on D-Wave 2000Q.
% \hl{add gpu-based CDCL solver.}
}
\vspace{-0.2cm}
\label{tab:speed_noise}
\renewcommand\arraystretch{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll}
\toprule

\textbf{} & \makecell[l]{\textbf{Minisat~\cite{sorensson2005minisat}} \\ \textbf{time (ms)}} &  \makecell[l]{\textbf{Kissat~\cite{cherif2021kissat}} \\ \textbf{time (ms)}} & \makecell[l]{\textbf{HyQSAT} \\ \textbf{time (ms)}} & \makecell[l]{\textbf{Speedup} \\ \textbf{(Minisat)}} & \makecell[l]{\textbf{Speedup} \\ \textbf{(Kissat)}} &\makecell[l]{\textbf{\#Iteration} \\ \textbf{variance}} \\
\midrule
\textbf{GC1} & 7.08 & 9.60 & 5.45 & 2.19 & 1.86 & 0.93  \\
\textbf{GC2} & 12.09 & 17.29 & 5.48 & 1.92 & 2.45 &0.93 \\
\textbf{GC3} & 27.1 & 30.95 & 12.52 & 2.61 & 3.31 &1.04 \\

\textbf{CFA} & 5.03 & 11.66 & 3.03 & 1.76 & 3.26 &5.46 \\
\textbf{BP} & 1.40 & 3.23 & 1.67 & 0.81  & 3.01 &0.49 \\

\textbf{II} & 1.48 & 4.18 & 1.58 & 0.89 & 3.53 &1.53 \\

% \textbf{\hl{IF}} & 582.92  & 1249.12 & 292.12 & 5.89  & 12.62 &2.41\\
\textbf{IF1} & 582.92  & 1249.12  & 292.13   & 5.89 & 12.62 & 2.41 \\
\textbf{IF2} & 34322.7 & 30137.88 & 12451.43 & 1.91 & 3.14  &  1.37 \\
\textbf{CRY} & 0.22    & 0.88     & 0.12     & 1.48 & 5.90   &  1.16    \\
% \textbf{SCH} & 29.84   & 32.34    & 13.63    & 1.52  & 2.32   &  0.74   \\
  
\textbf{AI1} & 20.00 & 39.38 & 5.97 & 5.32 & 8.82 &1.01 \\
\textbf{AI2} & 72.41 & 130.99 & 36.93 & 2.86 & 7.88 &1.27 \\
\textbf{AI3} & 180.72 & 196.68 & 82.88 & 3.72 & 4.82 &0.60 \\
\textbf{AI4} & 494.63  &318.17 & 204.05 & 4.69 & 4.38 &0.98\\
\textbf{AI5} & 1650.92 & 1307.23 & 828.8 & 5.33 & 3.71 &1.42 \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \caption{
% The running time comparison between CDCL on Intel E5 CPU and HyQSAT on D-Wave 2000Q. \hl{add gpu-based CDCL solver.}
% }
% \vspace{-0.2cm}
% \label{tab:speed_noise}
% \renewcommand\arraystretch{1.5}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|lllll}
% \toprule

% \textbf{} & \makecell[l]{\textbf{CDCL time} \\ \textbf{(ms)}} & \makecell[l]{\textbf{HyQSAT} \\ \textbf{time (ms)}} & \makecell[l]{\textbf{HyQSAT} \\ \textbf{speedup}} & \makecell[l]{\textbf{\#Iteration} \\ \textbf{variance}} & \makecell[l]{\textbf{Kissat} \\ \textbf{time (ms)}} \\
% \midrule
% \textbf{GC1} & $7.08^{+21.84}_{-6.78}$ & $5.45^{+9.40}_{-4.35}$ & $2.19^{+9.28}_{-1.18}$ & 0.93  & $7.85^{+7.41}_{-5.60}$\\
% \textbf{GC2} & $12.09^{+30.73}_{-10.89}$ & $5.48^{+26.03}_{-5.14}$ & $1.92^{+3.78}_{-1.01}$ & 0.93 & $13.60^{+62.80}_{-10.50}$ \\
% \textbf{GC3} & $27.1^{+97.68}_{-23.89}$ & $12.52^{+93.78}_{-12.15}$ & $2.61^{+12.53}_{-1.62}$ & 1.04 & $25.07^{+65.97}_{-22.35}$\\

% \textbf{CFA} & $5.03^{+4.17}_{-4.17}$ & $3.03^{+4.28}_{-2.38}$ &$1.76^{+1.52}_{-1.12}$ & 5.46 & $11.66^{+7.09}_{-7.09}$\\
% \textbf{BP} & $1.40^{+0.87}_{-0.86}$ & $1.67^{+0.96}_{-1.04}$ & $0.81^{+0.05}_{-0.05}$  & 0.49 & $4.84^{+6.66}_{-3.13}$\\
% % 

% \textbf{II} & $1.48^{+13.46}_{-1.34}$ & $1.58^{+4.45}_{-1.23}$ & $0.89^{+7.66}_{-0.75}$  & 1.53 & $5.85^{+6.84}_{-3.40}$\\

% \textbf{IF} & $582.92^{+16155.67}_{-582.58}$ & $292.12^{+8124.56}_{-291.96}$ & $5.89^{+26.66}_{-4.25}$  & 2.41 & \hl{??}\\

% \textbf{AI1} & $20.00^{+32.98}_{-17.42}$ & $5.97^{+20.84}_{-5.62}$ & $5.32^{+15.21}_{-3.70}$ & 1.01 & $28.63^{+77.20}_{-26.68}$\\
% \textbf{AI2} & $72.41^{+160.07}_{-66.06}$ & $36.93^{+115.60}_{-34.66}$ & $2.86^{+9.34}_{-1.06}$ & 1.27 &$89.43^{+397.53}_{-83.08}$\\
% \textbf{AI3} & $180.72^{+696.92}_{-156.74}$ & $82.88^{+497.80}_{-72.34}$ & $3.72^{+16.00}_{-2.71}$ & 0.60 & $111.93^{+473.61}_{-100.34}$\\
% \textbf{AI4} & $494.63^{+1023.28}_{-474.20}$ & $204.05^{+654.67}_{-195.49}$ & $4.69^{+50.27}_{-3.61}$ & 0.98 & $163.08^{+535.99}_{-148.94}$\\
% \textbf{AI5} & $1,772.02^{+2091.50}_{-1740.41}$ & $828.8^{+2595.30}_{-808.56}$ & $5.33^{+32.94}_{-4.39}$ & 1.42 &$637.73^{+1780.65}_{-561.47}$\\
% \bottomrule
% \end{tabular}
% }
% \vspace{-0.4cm}
% \end{table}


% \begin{table}[t]
% \centering
% \footnotesize
% \caption{
% The running time comparison between CDCL on Intel E5 CPU and HyQSAT on D-Wave 2000Q. \hl{add gpu-based CDCL solver.}
% }
% \vspace{-0.2cm}
% \label{tab:speed_noise}
% \renewcommand\arraystretch{1.5}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|lllll}
% \toprule
% % \textbf{ Benchmark & CDCL time (ms) & \makecell[l]{Our method \\ time (ms)} & \makecell[l]{Our method \\ speedup} & \makecell[l]{\#Iteration \\ variation} }\\
% \textbf{} & \makecell[l]{\textbf{CDCL time} \\ \textbf{(ms)}} & \makecell[l]{\textbf{HyQSAT} \\ \textbf{time (ms)}} & \makecell[l]{\textbf{HyQSAT} \\ \textbf{speedup}} & \makecell[l]{\textbf{\#Iteration} \\ \textbf{variance}} & \makecell[l]{\textbf{Kissat} \\ \textbf{time (ms)}} \\
% \midrule
% \textbf{GC1} & $7.08^{+21.84}_{-6.78}$ & $5.45^{+9.40}_{-4.35}$ & $2.19^{+9.28}_{-1.18}$ & 0.93  & $7.85^{+7.41}_{-5.60}$\\
% \textbf{GC2} & $12.09^{+30.73}_{-10.89}$ & $5.48^{+26.03}_{-5.14}$ & $1.92^{+3.78}_{-1.01}$ & 0.93 & $13.60^{+62.80}_{-10.50}$ \\
% \textbf{GC3} & $27.1^{+97.68}_{-23.89}$ & $12.52^{+93.78}_{-12.15}$ & $2.61^{+12.53}_{-1.62}$ & 1.04 & $25.07^{+65.97}_{-22.35}$\\

% \textbf{CFA} & $5.03^{+4.17}_{-4.17}$ & $3.03^{+4.28}_{-2.38}$ &$1.76^{+1.52}_{-1.12}$ & 5.46 & $11.66^{+7.09}_{-7.09}$\\
% \textbf{BP} & $1.40^{+0.87}_{-0.86}$ & $1.67^{+0.96}_{-1.04}$ & $0.81^{+0.05}_{-0.05}$  & 0.49 & $4.84^{+6.66}_{-3.13}$\\
% % 

% \textbf{II} & $1.48^{+13.46}_{-1.34}$ & $1.58^{+4.45}_{-1.23}$ & $0.89^{+7.66}_{-0.75}$  & 1.53 & $5.85^{+6.84}_{-3.40}$\\

% \textbf{IF} & $582.92^{+16155.67}_{-582.58}$ & $292.12^{+8124.56}_{-291.96}$ & $5.89^{+26.66}_{-4.25}$  & 2.41 & \hl{??}\\

% \textbf{AI1} & $20.00^{+32.98}_{-17.42}$ & $5.97^{+20.84}_{-5.62}$ & $5.32^{+15.21}_{-3.70}$ & 1.01 & $28.63^{+77.20}_{-26.68}$\\
% \textbf{AI2} & $72.41^{+160.07}_{-66.06}$ & $36.93^{+115.60}_{-34.66}$ & $2.86^{+9.34}_{-1.06}$ & 1.27 &$89.43^{+397.53}_{-83.08}$\\
% \textbf{AI3} & $180.72^{+696.92}_{-156.74}$ & $82.88^{+497.80}_{-72.34}$ & $3.72^{+16.00}_{-2.71}$ & 0.60 & $111.93^{+473.61}_{-100.34}$\\
% \textbf{AI4} & $494.63^{+1023.28}_{-474.20}$ & $204.05^{+654.67}_{-195.49}$ & $4.69^{+50.27}_{-3.61}$ & 0.98 & $163.08^{+535.99}_{-148.94}$\\
% \textbf{AI5} & $1,772.02^{+2091.50}_{-1740.41}$ & $828.8^{+2595.30}_{-808.56}$ & $5.33^{+32.94}_{-4.39}$ & 1.42 &$637.73^{+1780.65}_{-561.47}$\\
% \bottomrule
% \end{tabular}
% }
% \vspace{-0.4cm}
% \end{table}



% \begin{table}[]
% \centering
% \footnotesize
% \caption{The comparison of the iteration number of noise-free simulation and real world QA.}
% \label{tab:compare_itr}
% \begin{tabular}{cccc}
% \toprule
% % 
% Benchmark & Noise-free & Noise &   \makecell[l]{\#Iteration \\ variation} \\
% \midrule
% Flat150-360 & 179.84     & 166.88   & 0.93              \\
% Flat175-417 & 238.76     & 222.14   & 0.93              \\
% Flat200-479 & 414.86     & 429.80   & 1.04              \\
% bf          & 149.50     & 817.00   & 5.46              \\
% II          & 113.58     & 55.25    & 0.49              \\
% UF150-645   & 642.21     & 979.60   & 1.53              \\
% UF175-753   & 2953.72    & 2973.43  & 1.01              \\
% UF200-860   & 5416.84    & 6864.88  & 1.27              \\
% UF225-960   & 14133.00   & 8417.78  & 0.60              \\
% UF250-1065  & 50202.72   & 49176.00 & 0.98              \\
% Average     & 7444.50    & 7010.28  & 1.42              \\
% \bottomrule
% \end{tabular}
% \end{table}
% \hl{merge table III}

